Read, Watch and Scream! Sound Generation from Text and Video

Despite the impressive progress of multimodal generative models, video-to-audio generation still suffers from limited performance and limits the flexibility to prioritize sound synthesis for specific objects within the scene. Conversely, text-to-audio generation methods generate high-quality audio but pose challenges in ensuring comprehensive scene depiction and time-varying control. To tackle these challenges, we propose a novel video-and-text-to-audio generation method, called \ours, where video serves as a conditional control for a text-to-audio generation model. Especially, our method estimates the structural information of sound (namely, energy) from the video while receiving key content cues from a user prompt. We employ a well-performing text-to-audio model to consolidate the video control, which is much more efficient for training multimodal diffusion models with massive triplet-paired (audio-video-text) data. In addition, by separating the generative components of audio, it becomes a more flexible system that allows users to freely adjust the energy, surrounding environment, and primary sound source according to their preferences. Experimental results demonstrate that our method shows superiority in terms of quality, controllability, and training efficiency. Code and demo are available at https://naver-ai.github.io/rewas.

==> src/aaai_reproducitibility.tex <==

This paper:

\begin{itemize}
    \item{Includes a conceptual outline and/or pseudocode description of AI methods introduced }(yes/partial/no/NA)
    \begin{itemize}
    \item{\textbf{Answer}: partial}
    % \item{\textbf{Justification}: There is no pseudocode. However, we provided a conceptual outline as Figures.}
    \end{itemize}
    \item{Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results (yes/no)}
    \begin{itemize}
    \item{\textbf{Answer}: yes}
    % \item{\textbf{Justification}: We clearly delineate statements that are opinions, hypothesis, and speculation.}
    \end{itemize}
    \item{Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper (yes/no)} % not sure
    \begin{itemize}
    \item{\textbf{Answer}: yes}
    % \item{\textbf{Justification}: We clearly provided all necessary references to ensure that unfamiliar readers can easily access the relevant background information.}
    \end{itemize}

 % \end{itemize}


\item{Does this paper make theoretical contributions? (yes/no)}
\begin{itemize}
    \item{\textbf{Answer}: no}
    % \item{\textbf{Justification}: We did not make theoretical contributions.}
\end{itemize}
    
% If yes, please complete the list below.

% \begin{itemize}
% \item{All assumptions and restrictions are stated clearly and formally. (yes/partial/no)}
% \item{All novel claims are stated formally (e.g., in theorem statements). (yes/partial/no)}
% \item{Proofs of all novel claims are included. (yes/partial/no)}
% \item{Proof sketches or intuitions are given for complex and/or novel results. (yes/partial/no)}
% \item{Appropriate citations to theoretical tools used are given. (yes/partial/no)}
% \item{All theoretical claims are demonstrated empirically to hold. (yes/partial/no/NA)}
% \item{All experimental code used to eliminate or disprove claims is included. (yes/no/NA)}
% \item{}
% \end{itemize}

\item{Does this paper rely on one or more datasets?(yes/no)}
\begin{itemize}
    \item{\textbf{Answer}: yes}
    % \item{\textbf{Justification}: We relies on two datasets.}
\end{itemize}



% If yes, please complete the list below.
\begin{itemize}
\item{A motivation is given for why the experiments are conducted on the selected datasets (yes/partial/no/NA)}
\begin{itemize}
    \item{\textbf{Answer}: yes}
    % \item{\textbf{Justification}: We provided detailed explanations for each dataset and the reasons behind our selection.}
\end{itemize}
\item{All novel datasets introduced in this paper are included in a data appendix. (yes/partial/no/NA)}
\begin{itemize}
    \item{\textbf{Answer}: NA}
    % \item{\textbf{Justification}: We did not introduce novel datasets.}
\end{itemize}
\item{All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes/partial/no/NA)}
\begin{itemize}
    \item{\textbf{Answer}: NA}
    % \item{\textbf{Justification}: We did not introduce novel datasets.}
\end{itemize}
\item{All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. (yes/no/NA)}
\begin{itemize}
    \item{\textbf{Answer}: yes}
    % \item{\textbf{Justification}: We appropriately cited all the datasets we used.}
\end{itemize}
\item{All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. (yes/partial/no/NA)}
\begin{itemize}
    \item{\textbf{Answer}: yes}
    % \item{\textbf{Justification}: We used publicly available datasets.}
\end{itemize}
\item{All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. (yes/partial/no/NA)}
\begin{itemize}
    \item{\textbf{Answer}: NA}
    % \item{\textbf{Justification}: We did not use any non-publicly available dataset.}
\end{itemize}
\end{itemize}


\item{Does this paper include computational experiments? (yes/no)}
\begin{itemize}
    \item{\textbf{Answer}: yes}
    % \item{\textbf{Justification}: We included experiments that require model training.}
\end{itemize}
% \begin{itemize}
% If yes, please complete the list below.
\begin{itemize}
\item{Any code required for pre-processing data is included in the appendix. (yes/partial/no).}
\begin{itemize}
    \item{\textbf{Answer}: yes}
    % \item{\textbf{Justification}: We included the detailed method of data pre-processing in the appendix.}
\end{itemize}

\item{All source code required for conducting and analyzing the experiments is included in a code appendix. (yes/partial/no)}
\begin{itemize}
    \item{\textbf{Answer}: yes}
    % \item{\textbf{Justification}: We will provide source code in a code appendix.}
\end{itemize}
\item{All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes/partial/no)}
\begin{itemize}
    \item{\textbf{Answer}: yes}
    % \item{\textbf{Justification}: The code will be made publicly available.}
\end{itemize}

\item{All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from (yes/partial/no)}
\begin{itemize}
    \item{\textbf{Answer}: yes}
    % \item{\textbf{Justification}: The code references will be cited appropriately.}
\end{itemize}

\item{If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. (yes/partial/no/NA)}
\begin{itemize}
    \item{\textbf{Answer}: yes}
    % \item{\textbf{Justification}: The code appendix will include a default seed for the replication of results.}
\end{itemize}


\item{This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. (yes/partial/no)}
\begin{itemize}
    \item{\textbf{Answer}: partial}
    % \item{\textbf{Justification}: GPU models will be illustrated in the appendix. Relevant software libraries will also be provided in the code appendix.}
\end{itemize}

\item{This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. (yes/partial/no)}
\begin{itemize}
    \item{\textbf{Answer}: yes}
    % \item{\textbf{Justification}: In the Experiments section, we described the evaluation metrics and explained the motivation for choosing these metrics.}
\end{itemize}

\item{This paper states the number of algorithm runs used to compute each reported result. (yes/no)}
\begin{itemize}
    \item{\textbf{Answer}: no}
    % \item{\textbf{Justification}: We did not state the number of algorithm runs, but we clearly specified the time required for training the algorithm.}
\end{itemize}

\item{Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. (yes/no)}
\begin{itemize}
    \item{\textbf{Answer}: no}
    % \item{\textbf{Justification}: We did not go beyond single-dimensional summaries of performance. However, we fixed the seed so that the reader can reproduce the same results.}
\end{itemize}

\item{The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). (yes/partial/no)}
\begin{itemize}
    \item{\textbf{Answer}: partial}
    % \item{\textbf{Justification}: We conducted an ablation study to evaluate the model's improvement or degradation under different settings, using appropriate metrics.}
\end{itemize}

\item{This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. (yes/partial/no/NA)}
\begin{itemize}
    \item{\textbf{Answer}: partial}
    % \item{\textbf{Justification}: We included most of the parameters we used. Any missing parameters related to diffusion can be found in the code appendix.}
\end{itemize}

\item{This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. (yes/partial/no/NA)}
\begin{itemize}
    \item{\textbf{Answer}: NA}
    % \item{\textbf{Justification}: We did not specify the range of values tested for each parameter, as it is not directly related to our main contribution.}
\end{itemize}
\end{itemize}
\end{itemize}
